Relaxing Integrity Requirements for Attack-Resilient Cyber-Physical Systems

The increase in network connectivity has also resulted in several high-profile attacks on cyber-physical systems. An attacker that manages to access a local network could remotely affect control performance by tampering with sensor measurements delivered to the controller. Recent results have shown that with network-based attacks, such as Man-in-the-Middle attacks, the attacker can introduce an unbounded state estimation error if measurements from a suitable subset of sensors contain false data when delivered to the controller. While these attacks can be addressed with the standard cryptographic tools that ensure data integrity, their continuous use would introduce significant communication and computation overhead. Consequently, we study effects of intermittent data integrity guarantees on system performance under stealthy attacks. We consider linear estimators equipped with a general type of residual-based intrusion detectors (including $\chi^2$ and SPRT detectors), and show that even when integrity of sensor measurements is enforced only intermittently, the attack impact is significantly limited; specifically, the state estimation error is bounded or the attacker cannot remain stealthy. Furthermore, we present methods to: (1) evaluate the effects of any given integrity enforcement policy in terms of reachable state-estimation errors for any type of stealthy attacks, and (2) design an enforcement policy that provides the desired estimation error guarantees under attack. Finally, on three automotive case studies we show that even with less than 10% of authenticated messages we can ensure satisfiable control performance in the presence of attacks.

==> bio.tex <==
% !TEX root = IntegrityRequirements_NewRegionsMethod_2017.tex

%\vspace{-14px}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Jovanov.jpg}}]
{Ilija Jovanov} received the Dipl. Ing. and M.S. degrees in electrical engineering from the University of Belgrade, Serbia, in 2014 and 2015, respectively.

He is currently a Ph.D. student at Department of Electrical and Computer Engineering, Pratt School of Electrical Engineering, Duke University, where he focuses on attack resilient control of cyber-physical systems.

\end{IEEEbiography}


%\vspace{-14px}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Pajic.jpg}}]{Miroslav Pajic}
 (S'06-M'13) received the Dipl. Ing. and M.S. degrees in electrical engineering from the University of Belgrade, Serbia, in 2003 and 2007, respectively, and the M.S. and Ph.D. degrees in electrical engineering from the University of Pennsylvania, Philadelphia, in 2010 and 2012, respectively.

He is currently an Assistant Professor in the Department of Electrical and Computer Engineering at Duke University. He also holds a secondary appointment in the Computer Science Department. Prior to joining Duke, Dr. Pajic was a Postdoctoral Researcher in the PRECISE Center, University of Pennsylvania. His research interests focus on the design and analysis of cyber-physical systems and in particular distributed/networked control systems, embedded systems, and high-confidence control system.

Dr. Pajic received various awards including the NSF CAREER Award, ONR Young Investigator Program  Award, 2011 ACM SIGBED Frank Anger Memorial Award, the Joseph and Rosaline Wolf Best Dissertation Award from Penn Engineering, the Best Paper Awards at the 2014 ACM/IEEE International Conference on Cyber-Physical Systems (ICCPS) and 2017  ACM International Conference on Embedded Software (EMSOFT), as well as the Best Student Paper Award at the 2012 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS).
\end{IEEEbiography}


==> proofT3.tex <==
% !TEX root = IntegrityRequirements_NewRegionsMethod_2017.tex


\begin{proof}
{\color{red} ATTEMPT WITH MIXED OBSERVABILITY INDEX AND OLD APPROACH}
From~\eqref{eq:dEk} and~\eqref{eq:dZk} it follows that
	\begin{align}
		\label{eq:dEkLemma}
		\Delta \mathbf{e}_{k+f} &= \mathbf{A}\Delta \mathbf{e}_{k+f-1} - \mathbf{K}\Delta \mathbf{z}_{k+f}, \\
		\label{eq:dZkLemma}
		\Delta \mathbf{z}_{k+f} &= \mathbf{CA}\Delta \mathbf{e}_{k+f-1}+\mathbf{ a}_{k+f} 
	\end{align} %\IL{We discussed using this to show that we need to attack along specific eigenvectors. However...}
%From the theorem's assumptions it follows that $\|\mathbf{CA}\Delta \mathbf{e}_{k+f-1}\|_2$ is bounded. 
Since $\|\mathbf{K}\|_2$ is finite, and $\|\Delta \mathbf{z}_{k+f}\|_2\leq 1$ due to the stealthy attack constraint~\eqref{eqn:z_th}, then $\|\mathbf{K}\Delta \mathbf{z}_{k+f}\|_2 \leq\|\mathbf{K}\|_2\|\Delta \mathbf{z}_{k+f}\|_2$ is bounded. Thus, to show that $\|\Delta \mathbf{e}_{k+f}\|_2$ is bounded, it is sufficient to prove that $\|\mathbf{A}\Delta \mathbf{e}_{k+f-1}\|_2$ is bounded.

Let's assume the opposite -- i.e.,~that $\|\mathbf{A}\Delta \mathbf{e}_{k+f-1}\|_2$ is unbounded while $\|\mathbf{CA}\Delta\mathbf{e}_{k}\|_2,\dots,\|\mathbf{CA}\Delta\mathbf{e}_{k+f-1}\|_2$ are all bounded. From~\eqref{eq:dEkLemma} it follows that %\PA{Ilija, pls check}
%$$\mathbf{A}\Delta\mathbf{e}_{k+f-1} = \mathbf{A}^{f}\Delta\mathbf{e}_k-\mathbf{A}^{f-1}\mathbf{K}\Delta\mathbf{z}_{k+1}-\dots-\mathbf{AK}\Delta\mathbf{z}_{k+f-1}$$
%\vspace{-4pt}
$$\mathbf{A}\Delta\mathbf{e}_{k+f-1} = \mathbf{A}^{f}\Delta\mathbf{e}_k-\sum_{j=1}^{f-1}\mathbf{A}^{f-j}\mathbf{K}\Delta\mathbf{z}_{k+j}.$$

\noindent Given that $\|\Delta\mathbf{z}_{k+1}\|, \dots, \|\Delta\mathbf{z}_{k+f-1}\|$ are bounded due to the stealthy attack requirements, in order for $\mathbf{A}\Delta\mathbf{e}_{k+f-1}$ to be unbounded, $\mathbf{A}^{f}\Delta\mathbf{e}_k$ has to be unbounded as well.

{\color{red} \textbf{\textit{Case~I}}: $f$ is nullity index of $(\mathbf{C,A})$ 

Given that $\mathbf{CA}\Delta\mathbf{e}_{k+1}$ is bounded, this implies that $\mathbf{CA}(\mathbf{A}\Delta\mathbf{e}_k - \mathbf{K}\Delta\mathbf{z}_{k+1})$ has to be bounded too. However, as $\Delta\mathbf{z}_{k+1}$ has to be bounded due to the stealthiness condition, it follows that $\mathbf{CA}^2\Delta\mathbf{e}_k$ has to remain bounded. Similarly, we can show that this holds up to $\mathbf{CA}^f\Delta\mathbf{e}_k$. This condition can be stated as
\begin{equation}
	\underbrace{
	\begin{bmatrix}
		\mathbf{C} \\
		\mathbf{CA}\\
		\dots\\
		\mathbf{CA}^{f-1}
	\end{bmatrix}
	}_{\mathcal{O}_f}
	\mathbf{A}\Delta\mathbf{e}_k = \mathbf{w}_k,
\label{ObsIndexCond}
\end{equation}
where $\mathbf{w}_k$ represents some bounded vector. Given that $\mathcal{O}_f$ has full rank due to the definition of the observability index, it follows that $\mathbf{A}\Delta\mathbf{e}_k$ has to be bounded. However, since $f$ is finite and $\mathbf{A}$ has finite elements, then $\mathbf{A}^{f-1}\mathbf{A}\Delta\mathbf{e}_k$ must be bounded too. This contradicts assumption that $\mathbf{A}^{f}\Delta\mathbf{e}_k$ is unbounded, which concludes this case.
}

%On the other hand, %although the matrix A may not be diagonalizable in general%{\color{red} if we introduce following decomposition}
%, if we utilize the generalized eigenvectors of $\mathbf{A}$ as a base of $\mathbb{R}^n$
{\color{red} \textbf{\textit{Case~II}}: $f$ is $q_{un}$ 

Observe that $\mathbf{A}^f\Delta\mathbf{e}_k$ being unbounded implies that $\Delta\mathbf{e}_k$ has to be unbounded. If we utilize decomposition from Lemma~\ref{lemma:bound} %, and denote with $\lambda_i, i=1,...,l$ corresponding eigenvalues of $\mathbf{A}$, 
 it follows that
%, the estimation error can be specified as
%
%\vspace{-14pt}
%\begin{equation}
%\label{eqn:e_vs}
%\Delta \mathbf{e}_{k} = \alpha_1\mathbf{v}_1+\dots+\alpha_n\mathbf{v}_n,
%\end{equation}
%
%where $\alpha_i\in\mathbb{R}$, $\mathbf{v}_i$, $i=1,...,l$ are eigenvectors of $\mathbf{A}$, and $\mathbf{v}_i$, $i=l+1,...,n$ are remaining generalized eigenvectors of $\mathbf{A}$ 
%{\color{red} linearly independent unit vectors that span $\mathcal{N}(\mathbf{A})$ }\IL{Reviewer 2, comment2)}(i.e.,~vectors that are used to complete a base of $\mathbb{R}^n$).
%Given this representation, if we denote with $\lambda_i, i=1,...,l$ corresponding eigenvalues of $\mathbf{A}$, it follows that
%
\begin{equation}
\label{eqn:Afe}
%\mathbf{A}^{f}\Delta\mathbf{e}_k = \alpha_1\lambda_1^{f}\mathbf{v}_1+\dots+\alpha_l\lambda_l^{f}\mathbf{v}_l+\mathbf{A}^{f}(\alpha_{l+1}\mathbf{v}_{l+1}+\dots+\alpha_n\mathbf{v}_n).
\mathbf{A}^{f}\Delta\mathbf{e}_k = \mathbf{A}^{f}\sum_{i=1}^q\alpha_i\mathbf{v}_i + \mathbf{A}^{f}\mathbf{w}_k
\end{equation}
%\PA{n not l, right?}
%
}

{\color{red}
As shown in the lemma, given that $\Delta\mathbf{e}_k$ is unbounded, at least one $\alpha_i\rightarrow\infty$, and $\mathbf{v}_i$ are eigenvectors and generalized eigenvectors corresponding to unstable eigenvalues, while $\mathbf{w}_k$ is some bounded vector.} 
%{\color{red} Constraint on $i$ is imposed since $\mathbf{v}_{l+1},\dots,\mathbf{v}_{n}\in null(\mathbf{C})$, and thus $\alpha_{l+1},\dots,\alpha_{n}$ have no effect on the sum.}\IL{Reviewer 2, comment 2)}.
%
%Let us observe the case where $\alpha_i$-s are the infinite coefficients. 
%Following directly the approach {\color{red} from~\cite{kwon2014stealthy}
%,mo2010falseincsys
% used to prove the necessary part of Theorem~\ref{thm:PA}}\IL{Reviewer 2, comment 1)}
%{\color{red} in previous lemma, we show} that these $\alpha_i\rightarrow\infty$ can only be the gains of the eigenvectors that correspond to unstable eigenvalues.
%Without loss of generality, let's denote the indices of such unstable eigenvectors, i.e.,~for which $\alpha_i\rightarrow\infty$, as $i=1,\dots, r$, where $r\leq l$.
%\IL{I've put $l$ istead of $s_{un}$ here, since alphas next to the repeating eigenvalues can be infinite too.} 
%We impose this limit due to the conditions for perfect attacks presented in \cite{mo2010falseincsys,kwon2014stealthy}. \IL{If we look at the equations mentioned in previous comment, there is no obvious reason to use only \textbf{unstable} eigenvalues. Eigenvectors-$\Gamma$ relationship argument would make sense (and I use it in corollary proof), but why only the eigenvectors corresponding to unstable eigenvalues?}

{\color{red} In addition, let us denote $\mathbf{n}_k = \sum_{i=1}^q\alpha_i\mathbf{v}_i$, which captures unbounded part of the estimation error. }
%In addition, let's decompose  $\Delta \mathbf{e}_k$ into $\Delta \mathbf{e}_k=\mathbf{n}_k+\mathbf{w}_k$, where $\mathbf{n}_k = \alpha_1\mathbf{v}_1+\dots+\alpha_r\mathbf{v}_r$ and $\mathbf{w}_k = \alpha_{r+1}\mathbf{v}_{r+1}+\dots+\alpha_n\mathbf{v}_n$ capture the unbounded and bounded parts of the estimation error respectively. %\IL{Should we explicitly state that $\alpha_1,\dots,\alpha_r \rightarrow\infty$, while the other ones don't?} 
From the theorem's assumptions, it holds that
%
$\mathbf{CA}\Delta \mathbf{e}_{k} = \mathbf{CAn}_k+\mathbf{CAw}_k$ has to be bounded. %Since $\mathbf{CAw}_k$ is bounded, %due to the fact that the corresponding coefficients $\alpha_i$ are finite 
%it follows that $\mathbf{An}_k \in\mathcal{N}(\mathbf{C})$ (because $\mathbf{n}_k$ is unbounded{\color{red}, and $\mathbf{n}_k\cap\mathcal{N}(\mathbf{A})=\{\mathbf{0}\}$}\IL{Reviewer 2, comment 3)}). In order\IL{Unneeded text} to show that this holds, let us consider the $n_k$ in the following representation
Vector $\mathbf{n}_k$ can be rewritten as
%
\begin{equation}
	\mathbf{n}_k = \alpha_1\mathbf{v}_1+\dots+\alpha_r\mathbf{v}_q = \mathbf{V}\mathbf{\alpha}_{1..q},
\label{eq:decompn_k}
\end{equation}
where $\mathbf{V}=[\mathbf{v}_1|\dots|\mathbf{v}_q]$, $\mathbf{\alpha}_{1..q}=[\alpha_1~\dots~\alpha_q]^T$, {\color{red} and $\alpha_1\rightarrow\infty,~\dots,~\alpha_q\rightarrow\infty$}. 
%Given that $\mathbf{CAn}_k$ has to be bounded, this means that $\mathbf{CAV\alpha}_{1..r}$ is bounded. That is,  for the constant matrix $\mathbf{\Psi}=\mathbf{CAV}$ we have that $\mathbf{\Psi\alpha}_{1..r}$ is bounded. Given that all elements of vector $\mathbf{\alpha}_{1..r}$ are unbounded (i.e.~$\alpha_i\rightarrow\infty,~i\in\{1,\dots,r\}$), $\mathbf{\Psi\alpha}_{1..r}$ can be always bounded only if $\mathbf{\alpha}_{1..r}\in null(\mathbf{\Psi})$. 
%This in turn implies that $\mathbf{\Psi\alpha}_{1..r}=\mathbf{CAV\alpha}_{1..r}=\mathbf{CAn}_k=0$ which yields $\mathbf{An}_k\in null(\mathbf{C})$.
%$\mathbf{CAV\alpha}=0$. Finally, we obtain that $\mathbf{CAV\alpha}=\mathbf{CAn}_k=\mathbf{C}(\mathbf{An}_k)=0$ which shows that $\mathbf{An}_k\in null(\mathbf{C})$.
%\IL{Let me know if we should put this proof separately as an aside or something.}


In addition, from the theorem conditions $\|\mathbf{CA}\Delta\mathbf{e}_{k+1}\|_2$ is also bounded and
%
\begin{equation}
\begin{split}
	\mathbf{CA}\Delta\mathbf{e}_{k+1} &= \mathbf{CA}(\mathbf{A}\Delta\mathbf{e}_{k}-\mathbf{K}\Delta\mathbf{z}_{k+1}) \\
	&= \mathbf{CA^2n}_k + \mathbf{CA^2w}_k - \mathbf{CA}\mathbf{K}\Delta\mathbf{z}_{k+1}
\label{eq:bounds}
\end{split}
\end{equation}
%
Because $\mathbf{CA^2w}_k$ and $\mathbf{CA}\mathbf{K}\Delta\mathbf{z}_{k+1}$ are bounded,  this similarly imposes additional limitation on the attacker that $\mathbf{CA}^2\mathbf{n}_k$ has to be bounded as well
% -- using the same argument as in the previous paragraph this implies that $\mathbf{A}^2\mathbf{n}_k \in\mathcal{N}(\mathbf{C})$.
%
Similarly, this argument can be repeated to show that for the $f$ consecutive time-steps where $\mathbf{a}_k=\mathbf{0}$, the vectors $\mathbf{An}_k,\dots,\mathbf{A}^f\mathbf{n}_k$ all have to be bounded.%belong to the $\mathcal{N}(\mathbf{C})$.

To show that this cannot occur, consider vectors $\mathbf{b}_1,...,\mathbf{b}_f$, defined as $\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k$ -- i.e., %~as previously defined~
{\color{red}
\begin{equation}
\label{eqn:bk} 
%\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k = \alpha_1\lambda_1^{i}\mathbf{v}_1+\dots+\alpha_r\lambda_r^{i}\mathbf{v}_r, ~i=1,...,f.
\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k = \mathbf{VJ}^{i-1}\alpha_{1..q}
\end{equation}
where $\mathbf{J}$ represents a submatrix comprising of first $r$ rows and columns of Jordan form of matrix $\mathbf{A}$.
}

Consider % the equation 
\begin{equation}
\label{eqn:v21}
\gamma_1\mathbf{b}_1+\dots+\gamma_{\eta}\mathbf{b}_{\eta} = \sum_{i\in\mathcal{V}}^{}\alpha_i\lambda_i\mathbf{v}_i.
\end{equation}
Since the eigenvectors $\mathbf{v}_1,...,\mathbf{v}_r$ %have to be 
are linearly independent, as they are part of the considered $\mathbf{R}^n$  base, %due to the definition of the problem,  if we form a Vandermonde matrix once more, we get
it follows that
%
%\vspace{-4pt}
{\color{red}
\begin{equation}
\label{eqn:v2}
\begin{split}
diag(r\times(\alpha_{1..q})^T)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{P}_{\mathcal{J}}
 \begin{bmatrix} 
(J_1^{0})^T & \dots & (J_1^{f-1})^T \\
 \dots & \dots & \dots \\
 (J_q^{0})^T & \dots & (J_q^{f-1})^T 
 \end{bmatrix} \gamma_{1..f} = \\
= diag(\alpha_1\lambda_1,\dots,\alpha_q\lambda_q)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{1}_\mathcal{V},
\end{split}
\end{equation}
}
where $\mathbf{1}_\mathcal{V}\in\mathbb{R}^q$ is a sparse vector of 1s with support in $\mathcal{V}$.
{\color{red} \IL{We can show that this is full rank, as we did before.}. Let us multiply \eqref{eqn:v21} by $\mathbf{C}$ from left. Given that $\gamma$s are finite, as well as the fact that all $\mathbf{Cb}$s are bounded, it follows that sum on right hand side has to be bounded. However, that sum can be written as $\sum_{i\in\mathcal{V}}^{}\alpha_i\lambda_i\mathbf{v}_i = \lambda_1\mathbf{V}_\mathcal{V}\alpha_\mathcal{V}$, which would mean that $\mathbf{C}\mathbf{V}_\mathcal{V}\alpha_\mathcal{V}$ has to be bounded. We also know that $\mathbf{V}_\mathcal{V}\alpha_\mathcal{V}$ is a scaled eigenvector of $\mathbf{A}$ and that it is unbounded. However, this does not necessarily have to imply that it belongs to the null space of $\mathbf{C}$.}


%\PA{In essence, this means that both $\mathbf{An}_k$ and $\mathbf{A}^2\mathbf{n}_k$ have to belong to the null space of $\mathbf{C}$.}

%%%%We can write this as
%%%%\begin{multline}
%%%%	\mathbf{CA^2n}_k = \mathbf{CA}(\mathbf{An}_k) =\\ \mathbf{CA}(\alpha_1\lambda_1\mathbf{v}_1+\dots+\alpha_r\lambda_r\mathbf{v}_r) =\\ \mathbf{C}((\alpha_1\lambda^2_1\mathbf{v}_1+\dots+\alpha_r\lambda^2_r\mathbf{v}_r))
%%%%\label{eq:bounds2}
%%%%\end{multline}
%We can repeat this process in order to show that for $f$ consecutive integrity requirements $\mathbf{An}_k,\dots,\mathbf{A}^f\mathbf{n}_k$ have to belong to the null space of $\mathbf{C}$. We will consider two possible cases
%
%\vspace{4pt}
%\noindent
%\textbf{\textit{Case~I}} -- When $q_{un}>\hbox{nullity}(\mathbf{C})$ and number of distinct eigenvalues in $\lambda_1,\dots,\lambda_r$ is greater than $\hbox{nullity}(\mathbf{C})$: %\PA{define size of a vector space - be careful since this is a matrix. put in the notation section}
%\\In this case, from~\eqref{eqn:f} $f=\hbox{nullity}(\mathbf{C})+1$. 
%%what is f in this case?
%%
%%We start by case by introducing $\eta_I = size(null(\mathbf{C}))+1$. 
%Now consider vectors $\mathbf{b}_1,...,\mathbf{b}_f$, defined as $\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k$ -- i.e., %~as previously defined~
%{\color{red}
%\begin{equation}
%\label{eqn:bk} 
%%\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k = \alpha_1\lambda_1^{i}\mathbf{v}_1+\dots+\alpha_r\lambda_r^{i}\mathbf{v}_r, ~i=1,...,f.
%\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k = \mathbf{VJ}^{i-1}\alpha_{1..r}
%\end{equation}
%where $\mathbf{J}$ represents a submatrix comprising of first $r$ rows and columns of Jordan form of matrix $\mathbf{A}$.
%}
%
%As we have previously shown, vectors $\mathbf{b}_1,...,\mathbf{b}_f\in\mathcal{N}(\mathbf{C})$. Since the dimension %\PA{use dimension not size} 
%of $\mathcal{N}(\mathbf{C})$ is $f-1$, these vectors have to be linearly dependent; thus, there exist real coefficients $\gamma_1,...,\gamma_f\in\mathbb{R}$ such that 
%%
%%Trom the condition that $\mathbf{An}_k$ has to belong to $null(\mathbf{C})$, we have that the vector $\mathbf{b}_1=\alpha_1\lambda_1\mathbf{v}_1+\dots+\alpha_r\lambda_r\mathbf{v}_r$ has to belong to the $null(\mathbf{C})$. This implies that $size(null(\mathbf{C}))$ would not be able to be 0, since it contains at least one vector. 
%%From the condition that $\mathbf{A}^2\mathbf{n}_k$ has to belong to $null(\mathbf{C})$, we have that vector $\mathbf{b}_2=\alpha_1\lambda^2_1\mathbf{v}_1+\dots+\alpha_r\lambda^2_r\mathbf{v}_r$ has to belong to the $null(\mathbf{C})$. Since the equation $a\mathbf{b}_1 = \mathbf{b}_2$ has no solutions for $a$, then that would mean that these vectors are linearly independent. This further implies that $size(null(\mathbf{C}))$ has to be at least 2, in order to contain both of these vectors. If we iteratively apply the same logic for subsequent steps, from the condition that $\mathbf{A^{size(null(\mathbf{C}))+1}n}_k$ has to belong to $null(\mathbf{C})$, we have that the vector $\mathbf{b}_{size(null(\mathbf{C}))+1}=\alpha_1\lambda^{size(null(\mathbf{C}))}_1\mathbf{v}_1+\dots+\alpha_r\lambda^{size(null(\mathbf{C}))}_r\mathbf{v}_r$ has to belong to the $null(\mathbf{C})$. 
%%Let us observe the equation 
%%$$a_1\mathbf{b}_1+\dots+a_{size(null(\mathbf{C}))}\mathbf{b}_{size(null(\mathbf{C}))}+a_{size(null(\mathbf{C}))+1}\mathbf{b}_{size(null(\mathbf{C}))+1=0}$$ 
%%Let $size(null(\mathbf{C}))+1 = \eta$. Then we can write
%$\gamma_1\mathbf{b}_1+\dots+\gamma_f\mathbf{b}_f=0$ -- i.e.,~from~\eqref{eqn:bk} 
%%$$\gamma_1(\alpha_1\lambda_1\mathbf{v}_1+...+\alpha_r\lambda_r\mathbf{v}_r)+...+\gamma_f(\alpha_1\lambda_1^f\mathbf{v}_1+...+\alpha_r\lambda_r^f\mathbf{v}_r) = 0.$$
%{\color{red}
%$$ \gamma_1\mathbf{VJ}^0\alpha_{1..r} + \dots + \gamma_f\mathbf{VJ}^{f-1}\alpha_{1..r} = 0.$$
%Given that $\mathbf{V}$ is full rank, as its columns are linearly independent, we can simplify this equation as
%$$ \gamma_1\mathbf{J}^0\alpha_{1..r} + \dots + \gamma_f\mathbf{J}^{f-1}\alpha_{1..r} = 0.$$
%If $\mathbf{J}_j^i$ denotes $j$-th row vector of matrix $\mathbf{J}^i$, we can use this to rewrite the previous equation as
%$$ \sum_{i=1}^{f}\gamma_i \begin{bmatrix} J_1^{i-1}\alpha_{1..r} \\ \dots \\ J_r^{i-1}\alpha_{1..r} \end{bmatrix} =
% \sum_{i=1}^{f}\gamma_i \begin{bmatrix} (\alpha_{1..r})^T(J_1^{i-1})^T \\ \dots \\ (\alpha_{1..r})^T(J_r^{i-1})^T \end{bmatrix} = 0, $$
%or rather
%$$ \begin{bmatrix} 
%(\alpha_{1..r})^T(J_1^{0})^T & \dots & (\alpha_{1..r})^T(J_1^{f-1})^T \\
% \dots & \dots & \dots \\
% (\alpha_{1..r})^T(J_r^{0})^T & \dots & (\alpha_{1..r})^T(J_r^{f-1})^T 
% \end{bmatrix}
% \underbrace{
% \begin{bmatrix}
% \gamma_1 \\ \dots \\ \gamma_f
%\end{bmatrix}}_{\gamma_{1..f}}  = 0, $$
%which finally provides us with the following equation.
%$$ diag(r\times(\alpha_{1..r})^T)
%\underbrace{
% \begin{bmatrix} 
%(J_1^{0})^T & \dots & (J_1^{f-1})^T \\
% \dots & \dots & \dots \\
% (J_r^{0})^T & \dots & (J_r^{f-1})^T 
% \end{bmatrix} \gamma_{1..f}
% }_{\gamma_{J}} = 0 $$
%where $r\times(\alpha_{1..r})^T$ represents transpose of the vector $\alpha_{1..r}$ repeated $r$ times. Take note that $J_j^i$ will have entries that are always zero, that correspond to the entries unrelated to $j$-th eigenvalue. Given this property, if we denote $supp(\gamma_{J})=\mathcal{J}$, then $|supp(\gamma_{J})|=r$ from Jordan matrix properties, and following holds
%$$ diag(r\times(\alpha_{1..r})^T)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{P}_{\mathcal{J}}\gamma_{J} = 0. $$
%Following the same property, $diag(r\times(\alpha_{1..r})^T)\mathbf{P}_{\mathcal{J}}^\dagger$ cannot have rows that are equal to $\mathbf{0}^T$ making given product a full rank square matrix. Finally, let us keep only the rows of $\mathbf{P}_{\mathcal{J}}\gamma_{J}$ that correspond to the first element in Jordan matrix block (first element of an eigenvector chain). Then, we obtain
%}
%
%%Since $\mathbf{v}_1,\dots,\mathbf{v}_r$ are linearly independent %\PA{check} 
%%this can be satisfied only if 
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%the following equations are satisfied\PA{cut if space needed}
%%%%%%%%%%%%%%\begin{align*}
%%%%%%%%%%%%%%	a_1\alpha_1\lambda_1+\dots+a_\eta\alpha_1\lambda_1^f = 0\\
%%%%%%%%%%%%%%	a_1\alpha_2\lambda_2+\dots+a_\eta\alpha_2\lambda_2^f = 0\\
%%%%%%%%%%%%%%	\dots\\
%%%%%%%%%%%%%%	a_1\alpha_r\lambda_r+\dots+a_\eta\alpha_r\lambda_r^f = 0.
%%%%%%%%%%%%%%\end{align*}
%%%%%%%%%%%%%%%If we write this in matrix form, we obtain
%%%%%%%%%%%%%%%$$
%%%%%%%%%%%%%%%\begin{bmatrix}
%%%%%%%%%%%%%%%	\alpha_1\lambda_1 & \alpha_1\lambda_1^2 & \dots & \alpha_1\lambda_1^\eta \\
%%%%%%%%%%%%%%%	\alpha_2\lambda_2 & \alpha_2\lambda_2^2 & \dots & \alpha_2\lambda_2^\eta \\
%%%%%%%%%%%%%%%	\hdotsfor{4}\\
%%%%%%%%%%%%%%%	\alpha_r\lambda_r & \alpha_r\lambda_r^2 & \dots & \alpha_r\lambda_r^\eta 
%%%%%%%%%%%%%%%\end{bmatrix}
%%%%%%%%%%%%%%%\begin{bmatrix}
%%%%%%%%%%%%%%%	a_1 \\ a_2 \\ \dots \\ a_\eta
%%%%%%%%%%%%%%%\end{bmatrix} = \mathbf{0}
%%%%%%%%%%%%%%%$$
%%%%%%%%%%%%%%%That is
%%%%%%%%%%%%%%or in equivalent representation \PA{define diag}\PA{is it f below, not $\eta -1$}
%\vspace{-4pt}
%$$
%%diag(\alpha_1\lambda_1,\dots,\alpha_r\lambda_r)
%\underbrace{
%\begin{bmatrix}
%	1 & \lambda_1 & \dots & \lambda_1^{f-1} \\
%	1 & \lambda_2 & \dots & \lambda_2^{f-1} \\
%	\hdotsfor{4}\\
%	1 & \lambda_r & \dots & \lambda_r^{f-1} 
%\end{bmatrix}}_{\mathbf{V}(\lambda_1,...,\lambda_r) _{r\times f}}
%%\underbrace{
%%\begin{bmatrix}
%%	1 & \lambda_1 & \dots & \lambda_1^{f-1} \\
%%	1 & \lambda_2 & \dots & \lambda_2^{f-1} \\
%%	\hdotsfor{4}\\
%%	1 & \lambda_r & \dots & \lambda_r^{f-1} 
%%\end{bmatrix}_{r\times f}}_{\mathbf{V}(\lambda_1,...,\lambda_r) _{r\times f}}
%\cdot %\underbrace{
%\begin{bmatrix}
%	\gamma_1 \\ \gamma_2 \\ \dots \\ \gamma_f
%\end{bmatrix}%}_{\mathbf{\gamma}_{1..f}}
%= \mathbf{0}.
%$$
%Since $\lambda_1,...,\lambda_r$ are unstable (and thus nonzero), the above condition can be represented as ${\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times f}}\cdot{\mathbf{\gamma}_{1..f}}= \mathbf{0}$; 
%here, ${\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times f}}$ denotes a Vandermonde matrix. From the condition of the Case I, it follows that the  number of distinct eigenvalues in $\lambda_1,\dots,\lambda_r$ is greater than or equal to $f$, and thus the matrix is full rank~\cite{hom1991topics} -- i.e., 
%$$\hbox{rank}\left({\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times f}}\right)=f.$$
%%Since $\lambda_1,...,\lambda_r$ are unstable (and thus nonzero), the above condition can be represented as
%
%Therefore, the vector $\mathbf{\gamma}_{1..f}$ has to be $\mathbf{0}$, and the $f$ vectors $\mathbf{b}_1,...,\mathbf{b}_f$ %\in\hbox{null}(\mathbf{C})$ 
%are linearly independent while belonging to a vector space with dimension $f-1$ (i.e.,~$\mathcal{N}(\mathbf{C})$).
%%Which leads to
%%$$
%%\begin{bmatrix}
%%	1 & \lambda_1 & \dots & \lambda_1^{\eta-1} \\
%%	1 & \lambda_2 & \dots & \lambda_2^{\eta-1} \\
%%	\hdotsfor{4}\\
%%	1 & \lambda_r & \dots & \lambda_r^f 
%%\end{bmatrix}
%%\begin{bmatrix}
%%	a_1 \\ a_2 \\ \dots \\ a_\eta
%%\end{bmatrix} = \mathbf{0}
%%$$
%%Given that in this case number of distinct $\lambda_i$ values is greater than $\mathbf{b}_{size(null(\mathbf{C}))}$, and the matrix on the left hand side of the equation is a Vandermonde matrix, it will be full rank, producing trivial solution for $r=\eta$ or being overdetermined for $r>\eta$. This in turn shows that $\mathbf{b}_{size(null(\mathbf{C}))+1}$ is linearly independent from $\mathbf{b}_{1},\dots,\mathbf{b}_{size(null(\mathbf{C}))}$.
%%Since we know that $\mathbf{b}_{size(null(\mathbf{C}))+1}$ will have to belong to the null-space of $\mathbf{C}$, and that it's linearly independent from the other $\mathbf{b}$ vectors, this would require the $size(null(\mathbf{C}))$ to be equal to $size(null(\mathbf{C}))+1$. 
%This is a clear contradiction, and for this case, the theorem holds.
%
%\vspace{4pt}
%\noindent
%\textbf{\textit{Case~II}} -- When $q_{un}>\hbox{nullity}(\mathbf{C})$ and number of distinct eigenvalues in $\lambda_1,\dots,\lambda_r$ {\color{red} and sum of their algebraic and geometric multiplicity differences (denoted with $\eta$} is lower than $\hbox{nullity}(\mathbf{C})$, or $q_{un}\leq \hbox{nullity}(\mathbf{C})$:
%%Let us denote with $\eta$ the number of distinct eigenvalues in $\lambda_1,...,\lambda_r$.
% {\color{red} Take note that $\lambda_1,\dots,\lambda_r$ represent unstable eigenvalues that have corresponding infinite $\alpha_i$, so necessarily $\eta\leq q_{un}$. }\IL{Reviewer 4, comment 4)}From the condition of this case and the definition of $f$ it follows that $\eta \leq f$. 
%
%As in the previous case, let us form vectors $\mathbf{b}_1,\dots,\mathbf{b}_\eta \in \mathcal{N}(\mathbf{C})$, and let {\color{red}$\mathcal{V}=\{ i ~ |~ 1\leq i\leq r, \lambda_i=\lambda_1~and~\mathbf{v}_i~is~an~eigenvector \}$.} %\PA{check the range of i} 
%Consider % the equation 
%\begin{equation}
%\label{eqn:v21}
%\gamma_1\mathbf{b}_1+\dots+\gamma_{\eta}\mathbf{b}_{\eta} = \sum_{i\in\mathcal{V}}^{}\alpha_i\lambda_i\mathbf{v}_i.
%\end{equation}
%Since the eigenvectors $\mathbf{v}_1,...,\mathbf{v}_r$ %have to be 
%are linearly independent, as they are part of the considered $\mathbf{R}^n$  base, %due to the definition of the problem,  if we form a Vandermonde matrix once more, we get
%it follows that
%%
%%\vspace{-4pt}
%{\color{red}
%\begin{equation}
%\label{eqn:v2}
%\begin{split}
%%diag(\alpha_1\lambda_1,\dots,\alpha_r\lambda_r)
%%\begin{bmatrix}
%%	1 & \lambda_1 & \dots & \lambda_1^{\eta-1} \\
%%	1 & \lambda_2 & \dots & \lambda_2^{\eta-1} \\
%%	\hdotsfor{4}\\
%%	1 & \lambda_r & \dots & \lambda_r^{\eta-1} 
%%\end{bmatrix}
%%\begin{bmatrix}
%%	\gamma_1 \\ \gamma_2 \\ \dots \\ \gamma_\eta
%%\end{bmatrix} =\\
%diag(r\times(\alpha_{1..r})^T)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{P}_{\mathcal{J}}
% \begin{bmatrix} 
%(J_1^{0})^T & \dots & (J_1^{f-1})^T \\
% \dots & \dots & \dots \\
% (J_r^{0})^T & \dots & (J_r^{f-1})^T 
% \end{bmatrix} \gamma_{1..f} = \\
%= diag(\alpha_1\lambda_1,\dots,\alpha_r\lambda_r)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{1}_\mathcal{V},
%\end{split}
%\end{equation}
%}
%where $\mathbf{1}_\mathcal{V}\in\mathbb{R}^r$ is a sparse vector of 1s with support in $\mathcal{V}$.
%%
%%Since there are $\eta$ distinct values in the $r$ unstable eigenvalues, then the rank of the Vandermonde matrix $\mathbf{V}(\lambda_1,...,\lambda_r) _{r\times \eta}$ in~\eqref{eqn:v2} is equal to~$\eta$.
%{\color{red}
%Using Vandermonde matrices similarly to Case I along with the properties of power of Jordan matrix introduced in previous lemma, it follows that matrix comprised of Jordan matrix rows has full rank.} Furthermore, 
%%$$\hbox{rank}\left([\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times \eta} ~|~ \mathbf{1}_\mathcal{V}]\right)=\eta.$$
%%rank of the same matrix augmented by $\mathbf{1}_\mathcal{V}$ is going to be equal to $\eta$ as well. 
%From Kronecker--Capelli theorem, %this implies 
%it follows that there exist a non-trivial solution $\gamma_1,...,\gamma_{\eta}$ to~\eqref{eqn:v2} and thus~\eqref{eqn:v21}. On the other hand, a linear combination of eigenvectors corresponding to the same eigenvalue is also an eigenvector; thus
%%\IL{I can throw in a proof for this, just let me know if needed.}
%vector $\mathbf{v}_{}=\sum_{i\in\mathcal{V}}^{}\alpha_i\lambda_i\mathbf{v}_i$ is an eigenvector of $\mathbf{A}$. This implies that an eigenvector $\mathbf{v}$ of matrix $\mathbf{A}$ belongs to the subspace spanned by $\mathbf{b}_1,\dots,\mathbf{b}_{\eta}$, which is a subset of the $\mathcal{N}(\mathbf{C})$. This contradicts the starting assumptions, since $(\mathbf{A},\mathbf{C})$ is observable, %\PA{make sure it's specified} 
%and in that case an eigenvector of $\mathbf{A}$ may not belong to the $\mathcal{N}(\mathbf{C})$. 
%
%This concludes the proof, since the highest $\eta$ that can occur in this case is $\min(\hbox{nullity}(\mathbf{C})+1,q_{un}) = f$. %so with $f$ consecutive integrity enforcements, at least $\eta$ enforcements will always occur. %\PA{check}%, which is the reason to use it as a limit.
\end{proof}




==> proofT3_old.tex <==
% !TEX root = IntegrityRequirements_NewRegionsMethod_2017.tex


\begin{proof}
{\color{red} OLD APPROACH}
From~\eqref{eq:dEk} and~\eqref{eq:dZk} it follows that
	\begin{align}
		\label{eq:dEkLemma}
		\Delta \mathbf{e}_{k+f} &= \mathbf{A}\Delta \mathbf{e}_{k+f-1} - \mathbf{K}\Delta \mathbf{z}_{k+f}, \\
		\label{eq:dZkLemma}
		\Delta \mathbf{z}_{k+f} &= \mathbf{CA}\Delta \mathbf{e}_{k+f-1}+\mathbf{ a}_{k+f} 
	\end{align} %\IL{We discussed using this to show that we need to attack along specific eigenvectors. However...}
%From the theorem's assumptions it follows that $\|\mathbf{CA}\Delta \mathbf{e}_{k+f-1}\|_2$ is bounded. 
Since $\|\mathbf{K}\|_2$ is finite, and $\|\Delta \mathbf{z}_{k+f}\|_2\leq 1$ due to the stealthy attack constraint~\eqref{eqn:z_th}, then $\|\mathbf{K}\Delta \mathbf{z}_{k+f}\|_2 \leq\|\mathbf{K}\|_2\|\Delta \mathbf{z}_{k+f}\|_2$ is bounded. Thus, to show that $\|\Delta \mathbf{e}_{k+f}\|_2$ is bounded, it is sufficient to prove that $\|\mathbf{A}\Delta \mathbf{e}_{k+f-1}\|_2$ is bounded.

Let's assume the opposite -- i.e.,~that $\|\mathbf{A}\Delta \mathbf{e}_{k+f-1}\|_2$ is unbounded while $\|\mathbf{CA}\Delta\mathbf{e}_{k}\|_2,\dots,\|\mathbf{CA}\Delta\mathbf{e}_{k+f-1}\|_2$ are all bounded. From~\eqref{eq:dEkLemma} it follows that %\PA{Ilija, pls check}
%$$\mathbf{A}\Delta\mathbf{e}_{k+f-1} = \mathbf{A}^{f}\Delta\mathbf{e}_k-\mathbf{A}^{f-1}\mathbf{K}\Delta\mathbf{z}_{k+1}-\dots-\mathbf{AK}\Delta\mathbf{z}_{k+f-1}$$
%\vspace{-4pt}
$$\mathbf{A}\Delta\mathbf{e}_{k+f-1} = \mathbf{A}^{f}\Delta\mathbf{e}_k-\sum_{j=1}^{f-1}\mathbf{A}^{f-j}\mathbf{K}\Delta\mathbf{z}_{k+j}.$$

\noindent Given that $\|\Delta\mathbf{z}_{k+1}\|, \dots, \|\Delta\mathbf{z}_{k+f-1}\|$ are bounded due to the stealthy attack requirements, in order for $\mathbf{A}\Delta\mathbf{e}_{k+f-1}$ to be unbounded, $\mathbf{A}^{f}\Delta\mathbf{e}_k$ has to be unbounded as well.

On the other hand, %although the matrix A may not be diagonalizable in general%{\color{red} if we introduce following decomposition}
%, if we utilize the generalized eigenvectors of $\mathbf{A}$ as a base of $\mathbb{R}^n$
{\color{red}if we utilize decomposition from~\eqref{eq:e_vs}, and denote with $\lambda_i, i=1,...,l$ corresponding eigenvalues of $\mathbf{A}$, it follows that}
%, the estimation error can be specified as
%
%\vspace{-14pt}
%\begin{equation}
%\label{eqn:e_vs}
%\Delta \mathbf{e}_{k} = \alpha_1\mathbf{v}_1+\dots+\alpha_n\mathbf{v}_n,
%\end{equation}
%
%where $\alpha_i\in\mathbb{R}$, $\mathbf{v}_i$, $i=1,...,l$ are eigenvectors of $\mathbf{A}$, and $\mathbf{v}_i$, $i=l+1,...,n$ are remaining generalized eigenvectors of $\mathbf{A}$ 
%{\color{red} linearly independent unit vectors that span $\mathcal{N}(\mathbf{A})$ }\IL{Reviewer 2, comment2)}(i.e.,~vectors that are used to complete a base of $\mathbb{R}^n$).
%Given this representation, if we denote with $\lambda_i, i=1,...,l$ corresponding eigenvalues of $\mathbf{A}$, it follows that
%
\begin{equation}
\label{eqn:Afe}
%\mathbf{A}^{f}\Delta\mathbf{e}_k = \alpha_1\lambda_1^{f}\mathbf{v}_1+\dots+\alpha_l\lambda_l^{f}\mathbf{v}_l+\mathbf{A}^{f}(\alpha_{l+1}\mathbf{v}_{l+1}+\dots+\alpha_n\mathbf{v}_n).
\mathbf{A}^{f}\Delta\mathbf{e}_k = \mathbf{A}^{f}\sum_{i=1}^n\alpha_i\mathbf{v}_i
\end{equation}
%\PA{n not l, right?}
%

For the norm of this sum to be unbounded (as there is only a finite number of elements in the sum), at least one $\alpha_i\rightarrow\infty$ such that $\lambda_i \neq 0$ {\color{red}and $1\leq i\leq l$. Constraint on $i$ is imposed since $\mathbf{v}_{l+1},\dots,\mathbf{v}_{n}\in null(\mathbf{C})$, and thus $\alpha_{l+1},\dots,\alpha_{n}$ have no effect on the sum.}\IL{Reviewer 2, comment 2)}.
%
%Let us observe the case where $\alpha_i$-s are the infinite coefficients. 
%Following directly the approach {\color{red} from~\cite{kwon2014stealthy}
%,mo2010falseincsys
% used to prove the necessary part of Theorem~\ref{thm:PA}}\IL{Reviewer 2, comment 1)}
{\color{red} in previous lemma, we show} that these $\alpha_i\rightarrow\infty$ can only be the gains of the eigenvectors that correspond to unstable eigenvalues.
Without loss of generality, let's denote the indices of such unstable eigenvectors, i.e.,~for which $\alpha_i\rightarrow\infty$, as $i=1,\dots, r$, where $r\leq l$.
%\IL{I've put $l$ istead of $s_{un}$ here, since alphas next to the repeating eigenvalues can be infinite too.} 
%We impose this limit due to the conditions for perfect attacks presented in \cite{mo2010falseincsys,kwon2014stealthy}. \IL{If we look at the equations mentioned in previous comment, there is no obvious reason to use only \textbf{unstable} eigenvalues. Eigenvectors-$\Gamma$ relationship argument would make sense (and I use it in corollary proof), but why only the eigenvectors corresponding to unstable eigenvalues?}


In addition, let's decompose  $\Delta \mathbf{e}_k$ into $\Delta \mathbf{e}_k=\mathbf{n}_k+\mathbf{w}_k$, where $\mathbf{n}_k = \alpha_1\mathbf{v}_1+\dots+\alpha_r\mathbf{v}_r$ and $\mathbf{w}_k = \alpha_{r+1}\mathbf{v}_{r+1}+\dots+\alpha_n\mathbf{v}_n$ capture the unbounded and bounded parts of the estimation error respectively. %\IL{Should we explicitly state that $\alpha_1,\dots,\alpha_r \rightarrow\infty$, while the other ones don't?} 
From the theorem's assumptions, it holds that
%
$\mathbf{CA}\Delta \mathbf{e}_{k} = \mathbf{CAn}_k+\mathbf{CAw}_k$ has to be bounded. Since $\mathbf{CAw}_k$ is bounded, %due to the fact that the corresponding coefficients $\alpha_i$ are finite 
it follows that $\mathbf{An}_k \in\mathcal{N}(\mathbf{C})$ (because $\mathbf{n}_k$ is unbounded{\color{red}, and $\mathbf{n}_k\cap\mathcal{N}(\mathbf{A})=\{\mathbf{0}\}$}\IL{Reviewer 2, comment 3)}). In order\IL{Unneeded text} to show that this holds, let us consider the $n_k$ in the following representation
%
\begin{equation}
	\mathbf{n}_k = \alpha_1\mathbf{v}_1+\dots+\alpha_r\mathbf{v}_r = \mathbf{V}\mathbf{\alpha}_{1..r},
\label{eq:decompn_k}
\end{equation}
where $\mathbf{V}=[\mathbf{v}_1|\dots|\mathbf{v}_r]$, $\mathbf{\alpha}_{1..r}=[\alpha_1~\dots~\alpha_r]^T$, {\color{red} and $\alpha_1\rightarrow\infty,~\dots,~\alpha_r\rightarrow\infty$}. Given that $\mathbf{CAn}_k$ has to be bounded, this means that $\mathbf{CAV\alpha}_{1..r}$ is bounded. That is,  for the constant matrix $\mathbf{\Psi}=\mathbf{CAV}$ we have that $\mathbf{\Psi\alpha}_{1..r}$ is bounded. Given that all elements of vector $\mathbf{\alpha}_{1..r}$ are unbounded (i.e.~$\alpha_i\rightarrow\infty,~i\in\{1,\dots,r\}$), $\mathbf{\Psi\alpha}_{1..r}$ can be always bounded only if $\mathbf{\alpha}_{1..r}\in null(\mathbf{\Psi})$. 
This in turn implies that $\mathbf{\Psi\alpha}_{1..r}=\mathbf{CAV\alpha}_{1..r}=\mathbf{CAn}_k=0$ which yields $\mathbf{An}_k\in null(\mathbf{C})$.
%$\mathbf{CAV\alpha}=0$. Finally, we obtain that $\mathbf{CAV\alpha}=\mathbf{CAn}_k=\mathbf{C}(\mathbf{An}_k)=0$ which shows that $\mathbf{An}_k\in null(\mathbf{C})$.
%\IL{Let me know if we should put this proof separately as an aside or something.}


In addition, from the theorem conditions $\|\mathbf{CA}\Delta\mathbf{e}_{k+1}\|_2$ is also bounded and
%
\begin{equation}
\begin{split}
	\mathbf{CA}\Delta\mathbf{e}_{k+1} &= \mathbf{CA}(\mathbf{A}\Delta\mathbf{e}_{k}-\mathbf{K}\Delta\mathbf{z}_{k+1}) \\
	&= \mathbf{CA^2n}_k + \mathbf{CA^2w}_k - \mathbf{CA}\mathbf{K}\Delta\mathbf{z}_{k+1}
\label{eq:bounds}
\end{split}
\end{equation}
%
Because $\mathbf{CA^2w}_k$ and $\mathbf{CA}\mathbf{K}\Delta\mathbf{z}_{k+1}$ are bounded,  this similarly imposes additional limitation on the attacker that $\mathbf{CA}^2\mathbf{n}_k$ has to be bounded as well -- using the same argument as in the previous paragraph this implies that $\mathbf{A}^2\mathbf{n}_k \in\mathcal{N}(\mathbf{C})$.
%
Similarly, this argument can be repeated to show that for the $f$ consecutive time-steps where $\mathbf{a}_k=\mathbf{0}$, the vectors $\mathbf{An}_k,\dots,\mathbf{A}^f\mathbf{n}_k$ all have to belong to the $\mathcal{N}(\mathbf{C})$.

To show that this cannot occur, we consider two cases:

%\PA{In essence, this means that both $\mathbf{An}_k$ and $\mathbf{A}^2\mathbf{n}_k$ have to belong to the null space of $\mathbf{C}$.}

%%%%We can write this as
%%%%\begin{multline}
%%%%	\mathbf{CA^2n}_k = \mathbf{CA}(\mathbf{An}_k) =\\ \mathbf{CA}(\alpha_1\lambda_1\mathbf{v}_1+\dots+\alpha_r\lambda_r\mathbf{v}_r) =\\ \mathbf{C}((\alpha_1\lambda^2_1\mathbf{v}_1+\dots+\alpha_r\lambda^2_r\mathbf{v}_r))
%%%%\label{eq:bounds2}
%%%%\end{multline}
%We can repeat this process in order to show that for $f$ consecutive integrity requirements $\mathbf{An}_k,\dots,\mathbf{A}^f\mathbf{n}_k$ have to belong to the null space of $\mathbf{C}$. We will consider two possible cases

\vspace{4pt}
\noindent
\textbf{\textit{Case~I}} -- When $q_{un}>\hbox{nullity}(\mathbf{C})$ and number of distinct eigenvalues in $\lambda_1,\dots,\lambda_r$ is greater than $\hbox{nullity}(\mathbf{C})$: %\PA{define size of a vector space - be careful since this is a matrix. put in the notation section}
\\In this case, from~\eqref{eqn:f} $f=\hbox{nullity}(\mathbf{C})+1$. 
%what is f in this case?
%
%We start by case by introducing $\eta_I = size(null(\mathbf{C}))+1$. 
Now consider vectors $\mathbf{b}_1,...,\mathbf{b}_f$, defined as $\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k$ -- i.e., %~as previously defined~
{\color{red}
\begin{equation}
\label{eqn:bk} 
%\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k = \alpha_1\lambda_1^{i}\mathbf{v}_1+\dots+\alpha_r\lambda_r^{i}\mathbf{v}_r, ~i=1,...,f.
\mathbf{b}_i=\mathbf{A}^{i}\mathbf{n}_k = \mathbf{VJ}^{i-1}\alpha_{1..r}
\end{equation}
where $\mathbf{J}$ represents a submatrix comprising of first $r$ rows and columns of Jordan form of matrix $\mathbf{A}$.
}

As we have previously shown, vectors $\mathbf{b}_1,...,\mathbf{b}_f\in\mathcal{N}(\mathbf{C})$. Since the dimension %\PA{use dimension not size} 
of $\mathcal{N}(\mathbf{C})$ is $f-1$, these vectors have to be linearly dependent; thus, there exist real coefficients $\gamma_1,...,\gamma_f\in\mathbb{R}$ such that 
%
%Trom the condition that $\mathbf{An}_k$ has to belong to $null(\mathbf{C})$, we have that the vector $\mathbf{b}_1=\alpha_1\lambda_1\mathbf{v}_1+\dots+\alpha_r\lambda_r\mathbf{v}_r$ has to belong to the $null(\mathbf{C})$. This implies that $size(null(\mathbf{C}))$ would not be able to be 0, since it contains at least one vector. 
%From the condition that $\mathbf{A}^2\mathbf{n}_k$ has to belong to $null(\mathbf{C})$, we have that vector $\mathbf{b}_2=\alpha_1\lambda^2_1\mathbf{v}_1+\dots+\alpha_r\lambda^2_r\mathbf{v}_r$ has to belong to the $null(\mathbf{C})$. Since the equation $a\mathbf{b}_1 = \mathbf{b}_2$ has no solutions for $a$, then that would mean that these vectors are linearly independent. This further implies that $size(null(\mathbf{C}))$ has to be at least 2, in order to contain both of these vectors. If we iteratively apply the same logic for subsequent steps, from the condition that $\mathbf{A^{size(null(\mathbf{C}))+1}n}_k$ has to belong to $null(\mathbf{C})$, we have that the vector $\mathbf{b}_{size(null(\mathbf{C}))+1}=\alpha_1\lambda^{size(null(\mathbf{C}))}_1\mathbf{v}_1+\dots+\alpha_r\lambda^{size(null(\mathbf{C}))}_r\mathbf{v}_r$ has to belong to the $null(\mathbf{C})$. 
%Let us observe the equation 
%$$a_1\mathbf{b}_1+\dots+a_{size(null(\mathbf{C}))}\mathbf{b}_{size(null(\mathbf{C}))}+a_{size(null(\mathbf{C}))+1}\mathbf{b}_{size(null(\mathbf{C}))+1=0}$$ 
%Let $size(null(\mathbf{C}))+1 = \eta$. Then we can write
$\gamma_1\mathbf{b}_1+\dots+\gamma_f\mathbf{b}_f=0$ -- i.e.,~from~\eqref{eqn:bk} 
%$$\gamma_1(\alpha_1\lambda_1\mathbf{v}_1+...+\alpha_r\lambda_r\mathbf{v}_r)+...+\gamma_f(\alpha_1\lambda_1^f\mathbf{v}_1+...+\alpha_r\lambda_r^f\mathbf{v}_r) = 0.$$
{\color{red}
$$ \gamma_1\mathbf{VJ}^0\alpha_{1..r} + \dots + \gamma_f\mathbf{VJ}^{f-1}\alpha_{1..r} = 0.$$
Given that $\mathbf{V}$ is full rank, as its columns are linearly independent, we can simplify this equation as
$$ \gamma_1\mathbf{J}^0\alpha_{1..r} + \dots + \gamma_f\mathbf{J}^{f-1}\alpha_{1..r} = 0.$$
If $\mathbf{J}_j^i$ denotes $j$-th row vector of matrix $\mathbf{J}^i$, we can use this to rewrite the previous equation as
$$ \sum_{i=1}^{f}\gamma_i \begin{bmatrix} J_1^{i-1}\alpha_{1..r} \\ \dots \\ J_r^{i-1}\alpha_{1..r} \end{bmatrix} =
 \sum_{i=1}^{f}\gamma_i \begin{bmatrix} (\alpha_{1..r})^T(J_1^{i-1})^T \\ \dots \\ (\alpha_{1..r})^T(J_r^{i-1})^T \end{bmatrix} = 0, $$
or rather
$$ \begin{bmatrix} 
(\alpha_{1..r})^T(J_1^{0})^T & \dots & (\alpha_{1..r})^T(J_1^{f-1})^T \\
 \dots & \dots & \dots \\
 (\alpha_{1..r})^T(J_r^{0})^T & \dots & (\alpha_{1..r})^T(J_r^{f-1})^T 
 \end{bmatrix}
 \underbrace{
 \begin{bmatrix}
 \gamma_1 \\ \dots \\ \gamma_f
\end{bmatrix}}_{\gamma_{1..f}}  = 0, $$
which finally provides us with the following equation.
$$ diag(r\times(\alpha_{1..r})^T)
\underbrace{
 \begin{bmatrix} 
(J_1^{0})^T & \dots & (J_1^{f-1})^T \\
 \dots & \dots & \dots \\
 (J_r^{0})^T & \dots & (J_r^{f-1})^T 
 \end{bmatrix} \gamma_{1..f}
 }_{\gamma_{J}} = 0 $$
where $r\times(\alpha_{1..r})^T$ represents transpose of the vector $\alpha_{1..r}$ repeated $r$ times. Take note that $J_j^i$ will have entries that are always zero, that correspond to the entries unrelated to $j$-th eigenvalue. Given this property, if we denote $supp(\gamma_{J})=\mathcal{J}$, then $|supp(\gamma_{J})|=r$ from Jordan matrix properties, and following holds
$$ diag(r\times(\alpha_{1..r})^T)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{P}_{\mathcal{J}}\gamma_{J} = 0. $$
Following the same property, $diag(r\times(\alpha_{1..r})^T)\mathbf{P}_{\mathcal{J}}^\dagger$ cannot have rows that are equal to $\mathbf{0}^T$ making given product a full rank square matrix. Finally, let us keep only the rows of $\mathbf{P}_{\mathcal{J}}\gamma_{J}$ that correspond to the first element in Jordan matrix block (first element of an eigenvector chain). Then, we obtain
}

%Since $\mathbf{v}_1,\dots,\mathbf{v}_r$ are linearly independent %\PA{check} 
%this can be satisfied only if 
%%%%%%%%%%%%%
%%%%%%%%%%%%%
%%%%%%%%%%%%%the following equations are satisfied\PA{cut if space needed}
%%%%%%%%%%%%%\begin{align*}
%%%%%%%%%%%%%	a_1\alpha_1\lambda_1+\dots+a_\eta\alpha_1\lambda_1^f = 0\\
%%%%%%%%%%%%%	a_1\alpha_2\lambda_2+\dots+a_\eta\alpha_2\lambda_2^f = 0\\
%%%%%%%%%%%%%	\dots\\
%%%%%%%%%%%%%	a_1\alpha_r\lambda_r+\dots+a_\eta\alpha_r\lambda_r^f = 0.
%%%%%%%%%%%%%\end{align*}
%%%%%%%%%%%%%%If we write this in matrix form, we obtain
%%%%%%%%%%%%%%$$
%%%%%%%%%%%%%%\begin{bmatrix}
%%%%%%%%%%%%%%	\alpha_1\lambda_1 & \alpha_1\lambda_1^2 & \dots & \alpha_1\lambda_1^\eta \\
%%%%%%%%%%%%%%	\alpha_2\lambda_2 & \alpha_2\lambda_2^2 & \dots & \alpha_2\lambda_2^\eta \\
%%%%%%%%%%%%%%	\hdotsfor{4}\\
%%%%%%%%%%%%%%	\alpha_r\lambda_r & \alpha_r\lambda_r^2 & \dots & \alpha_r\lambda_r^\eta 
%%%%%%%%%%%%%%\end{bmatrix}
%%%%%%%%%%%%%%\begin{bmatrix}
%%%%%%%%%%%%%%	a_1 \\ a_2 \\ \dots \\ a_\eta
%%%%%%%%%%%%%%\end{bmatrix} = \mathbf{0}
%%%%%%%%%%%%%%$$
%%%%%%%%%%%%%%That is
%%%%%%%%%%%%%or in equivalent representation \PA{define diag}\PA{is it f below, not $\eta -1$}
\vspace{-4pt}
$$
%diag(\alpha_1\lambda_1,\dots,\alpha_r\lambda_r)
\underbrace{
\begin{bmatrix}
	1 & \lambda_1 & \dots & \lambda_1^{f-1} \\
	1 & \lambda_2 & \dots & \lambda_2^{f-1} \\
	\hdotsfor{4}\\
	1 & \lambda_r & \dots & \lambda_r^{f-1} 
\end{bmatrix}}_{\mathbf{V}(\lambda_1,...,\lambda_r) _{r\times f}}
%\underbrace{
%\begin{bmatrix}
%	1 & \lambda_1 & \dots & \lambda_1^{f-1} \\
%	1 & \lambda_2 & \dots & \lambda_2^{f-1} \\
%	\hdotsfor{4}\\
%	1 & \lambda_r & \dots & \lambda_r^{f-1} 
%\end{bmatrix}_{r\times f}}_{\mathbf{V}(\lambda_1,...,\lambda_r) _{r\times f}}
\cdot %\underbrace{
\begin{bmatrix}
	\gamma_1 \\ \gamma_2 \\ \dots \\ \gamma_f
\end{bmatrix}%}_{\mathbf{\gamma}_{1..f}}
= \mathbf{0}.
$$
Since $\lambda_1,...,\lambda_r$ are unstable (and thus nonzero), the above condition can be represented as ${\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times f}}\cdot{\mathbf{\gamma}_{1..f}}= \mathbf{0}$; 
here, ${\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times f}}$ denotes a Vandermonde matrix. From the condition of the Case I, it follows that the  number of distinct eigenvalues in $\lambda_1,\dots,\lambda_r$ is greater than or equal to $f$, and thus the matrix is full rank~\cite{hom1991topics} -- i.e., 
$$\hbox{rank}\left({\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times f}}\right)=f.$$
%Since $\lambda_1,...,\lambda_r$ are unstable (and thus nonzero), the above condition can be represented as

Therefore, the vector $\mathbf{\gamma}_{1..f}$ has to be $\mathbf{0}$, and the $f$ vectors $\mathbf{b}_1,...,\mathbf{b}_f$ %\in\hbox{null}(\mathbf{C})$ 
are linearly independent while belonging to a vector space with dimension $f-1$ (i.e.,~$\mathcal{N}(\mathbf{C})$).
%Which leads to
%$$
%\begin{bmatrix}
%	1 & \lambda_1 & \dots & \lambda_1^{\eta-1} \\
%	1 & \lambda_2 & \dots & \lambda_2^{\eta-1} \\
%	\hdotsfor{4}\\
%	1 & \lambda_r & \dots & \lambda_r^f 
%\end{bmatrix}
%\begin{bmatrix}
%	a_1 \\ a_2 \\ \dots \\ a_\eta
%\end{bmatrix} = \mathbf{0}
%$$
%Given that in this case number of distinct $\lambda_i$ values is greater than $\mathbf{b}_{size(null(\mathbf{C}))}$, and the matrix on the left hand side of the equation is a Vandermonde matrix, it will be full rank, producing trivial solution for $r=\eta$ or being overdetermined for $r>\eta$. This in turn shows that $\mathbf{b}_{size(null(\mathbf{C}))+1}$ is linearly independent from $\mathbf{b}_{1},\dots,\mathbf{b}_{size(null(\mathbf{C}))}$.
%Since we know that $\mathbf{b}_{size(null(\mathbf{C}))+1}$ will have to belong to the null-space of $\mathbf{C}$, and that it's linearly independent from the other $\mathbf{b}$ vectors, this would require the $size(null(\mathbf{C}))$ to be equal to $size(null(\mathbf{C}))+1$. 
This is a clear contradiction, and for this case, the theorem holds.

\vspace{4pt}
\noindent
\textbf{\textit{Case~II}} -- When $q_{un}>\hbox{nullity}(\mathbf{C})$ and number of distinct eigenvalues in $\lambda_1,\dots,\lambda_r$ {\color{red} and sum of their algebraic and geometric multiplicity differences (denoted with $\eta$} is lower than $\hbox{nullity}(\mathbf{C})$, or $q_{un}\leq \hbox{nullity}(\mathbf{C})$:
%Let us denote with $\eta$ the number of distinct eigenvalues in $\lambda_1,...,\lambda_r$.
 {\color{red} Take note that $\lambda_1,\dots,\lambda_r$ represent unstable eigenvalues that have corresponding infinite $\alpha_i$, so necessarily $\eta\leq q_{un}$. }\IL{Reviewer 4, comment 4)}From the condition of this case and the definition of $f$ it follows that $\eta \leq f$. 

As in the previous case, let us form vectors $\mathbf{b}_1,\dots,\mathbf{b}_\eta \in \mathcal{N}(\mathbf{C})$, and let {\color{red}$\mathcal{V}=\{ i ~ |~ 1\leq i\leq r, \lambda_i=\lambda_1~and~\mathbf{v}_i~is~an~eigenvector \}$.} %\PA{check the range of i} 
Consider % the equation 
\begin{equation}
\label{eqn:v21}
\gamma_1\mathbf{b}_1+\dots+\gamma_{\eta}\mathbf{b}_{\eta} = \sum_{i\in\mathcal{V}}^{}\alpha_i\lambda_i\mathbf{v}_i.
\end{equation}
Since the eigenvectors $\mathbf{v}_1,...,\mathbf{v}_r$ %have to be 
are linearly independent, as they are part of the considered $\mathbf{R}^n$  base, %due to the definition of the problem,  if we form a Vandermonde matrix once more, we get
it follows that
%
%\vspace{-4pt}
{\color{red}
\begin{equation}
\label{eqn:v2}
\begin{split}
%diag(\alpha_1\lambda_1,\dots,\alpha_r\lambda_r)
%\begin{bmatrix}
%	1 & \lambda_1 & \dots & \lambda_1^{\eta-1} \\
%	1 & \lambda_2 & \dots & \lambda_2^{\eta-1} \\
%	\hdotsfor{4}\\
%	1 & \lambda_r & \dots & \lambda_r^{\eta-1} 
%\end{bmatrix}
%\begin{bmatrix}
%	\gamma_1 \\ \gamma_2 \\ \dots \\ \gamma_\eta
%\end{bmatrix} =\\
diag(r\times(\alpha_{1..r})^T)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{P}_{\mathcal{J}}
 \begin{bmatrix} 
(J_1^{0})^T & \dots & (J_1^{f-1})^T \\
 \dots & \dots & \dots \\
 (J_r^{0})^T & \dots & (J_r^{f-1})^T 
 \end{bmatrix} \gamma_{1..f} = \\
= diag(\alpha_1\lambda_1,\dots,\alpha_r\lambda_r)\mathbf{P}_{\mathcal{J}}^\dagger\mathbf{1}_\mathcal{V},
\end{split}
\end{equation}
}
where $\mathbf{1}_\mathcal{V}\in\mathbb{R}^r$ is a sparse vector of 1s with support in $\mathcal{V}$.
%
%Since there are $\eta$ distinct values in the $r$ unstable eigenvalues, then the rank of the Vandermonde matrix $\mathbf{V}(\lambda_1,...,\lambda_r) _{r\times \eta}$ in~\eqref{eqn:v2} is equal to~$\eta$.
{\color{red}
Using Vandermonde matrices similarly to Case I along with the properties of power of Jordan matrix introduced in previous lemma, it follows that matrix comprised of Jordan matrix rows has full rank.} Furthermore, 
%$$\hbox{rank}\left([\mathbf{V}(\lambda_1,...,\lambda_r)_{r\times \eta} ~|~ \mathbf{1}_\mathcal{V}]\right)=\eta.$$
%rank of the same matrix augmented by $\mathbf{1}_\mathcal{V}$ is going to be equal to $\eta$ as well. 
From Kronecker--Capelli theorem, %this implies 
it follows that there exist a non-trivial solution $\gamma_1,...,\gamma_{\eta}$ to~\eqref{eqn:v2} and thus~\eqref{eqn:v21}. On the other hand, a linear combination of eigenvectors corresponding to the same eigenvalue is also an eigenvector; thus
%\IL{I can throw in a proof for this, just let me know if needed.}
vector $\mathbf{v}_{}=\sum_{i\in\mathcal{V}}^{}\alpha_i\lambda_i\mathbf{v}_i$ is an eigenvector of $\mathbf{A}$. This implies that an eigenvector $\mathbf{v}$ of matrix $\mathbf{A}$ belongs to the subspace spanned by $\mathbf{b}_1,\dots,\mathbf{b}_{\eta}$, which is a subset of the $\mathcal{N}(\mathbf{C})$. This contradicts the starting assumptions, since $(\mathbf{A},\mathbf{C})$ is observable, %\PA{make sure it's specified} 
and in that case an eigenvector of $\mathbf{A}$ may not belong to the $\mathcal{N}(\mathbf{C})$. 

This concludes the proof, since the highest $\eta$ that can occur in this case is $\min(\hbox{nullity}(\mathbf{C})+1,q_{un}) = f$. %so with $f$ consecutive integrity enforcements, at least $\eta$ enforcements will always occur. %\PA{check}%, which is the reason to use it as a limit.
\end{proof}



